On the Gabriel quiver of extensions of Leibniz algebras

We compute the Gabriel quiver of simple objects in the category of bimodules over a simple Leibniz algebra and over the trivial $1$-dimensional Leibniz algebra. Vertices of the quiver are the classes of simple objects, arrows are given by the dimensions of Ext$^1$-groups.

==> extensions.tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da38621756976167587] 
\draw    (140,50) -- (218,50) ;
\draw [shift={(220,50)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da832360486693482] 
\draw    (260,50) -- (338,50) ;
\draw [shift={(340,50)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28584741488957444] 
\draw    (140,130) -- (218,130) ;
\draw [shift={(220,130)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9794527014152294] 
\draw    (250,130) -- (338,129.02) ;
\draw [shift={(340,129)}, rotate = 179.36] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9459660105492573] 
\draw    (240,60) -- (240,118) ;
\draw [shift={(240,120)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7013184147528526] 
\draw    (350,60) -- (350,120) ;
%Straight Lines [id:da013398067938281022] 
\draw    (360,62) -- (360,120) ;
%Straight Lines [id:da022418722168985994] 
\draw    (120,60) -- (120,120) ;
%Straight Lines [id:da14031143806284696] 
\draw    (130,60) -- (130,120) ;

% Text Node
\draw (121,42.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
% Text Node
\draw (231,42.4) node [anchor=north west][inner sep=0.75pt]    {$E_{1}$};
% Text Node
\draw (344,42.4) node [anchor=north west][inner sep=0.75pt]    {$A$};
% Text Node
\draw (121,122.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
% Text Node
\draw (228,122.4) node [anchor=north west][inner sep=0.75pt]    {$E_{2}$};
% Text Node
\draw (344,122.4) node [anchor=north west][inner sep=0.75pt]    {$A$};
% Text Node
\draw (251,82.4) node [anchor=north west][inner sep=0.75pt]    {$g$};


\end{tikzpicture}

